Segment Augmentation and Differentiable Ranking for Logo Retrieval

Logo retrieval is a challenging problem since the definition of similarity is more subjective compared to image retrieval tasks and the set of known similarities is very scarce. To tackle this challenge, in this paper, we propose a simple but effective segment-based augmentation strategy to introduce artificially similar logos for training deep networks for logo retrieval. In this novel augmentation strategy, we first find segments in a logo and apply transformations such as rotation, scaling, and color change, on the segments, unlike the conventional image-level augmentation strategies. Moreover, we evaluate whether the recently introduced ranking-based loss function, Smooth-AP, is a better approach for learning similarity for logo retrieval. On the large scale METU Trademark Dataset, we show that (i) our segment-based augmentation strategy improves retrieval performance compared to the baseline model or image-level augmentation strategies, and (ii) Smooth-AP indeed performs better than conventional losses for logo retrieval.

==> Albumentations_table.tex <==

% SK: Supp matt'a tasindi

==> ICPR2022 -- Logo Retrieval/Albumentations_table.tex <==

% SK: Supp matt'a tasindi

==> ICPR2022 -- Logo Retrieval/buyuk_tablo.tex <==
\begin{table*}[hbt!]
\centering
\caption{\label{tab:SmoothAP-DataAugmentation} Normalized Average Rank (NAR) and Recall@K values for data augmentation experiments with Smooth-AP Loss.}
 \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l l l l l | l l l l l l @{}}
\toprule
\textbf{} &
  \textbf{} &
  \textbf{Image Level} &
  \textbf{} &
   &
   & 
  \textbf{Segment Level} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
   \\ \midrule
\multicolumn{1}{c}{Resized Crop} &
  \multicolumn{1}{c}{Hor. Flip} &
  \multicolumn{1}{c}{Vert. Flip} &
  \multicolumn{1}{c}{Rotation} &
  \multicolumn{1}{c}{Color Jitter} &
  \multicolumn{1}{|c}{S. Color Change} &
  \multicolumn{1}{c}{S. Rotation} &
  \multicolumn{1}{c}{S. Removal} &
  \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
  \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
  \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
\multicolumn{8}{c}{\textit{Baseline}} &
  \multicolumn{1}{c}{0.102} &
  \multicolumn{1}{c}{0.310} &
  \multicolumn{1}{c}{0.536} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.046} &
  \multicolumn{1}{c}{0.339} &
  \multicolumn{1}{c}{0.581} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.049} &
  \multicolumn{1}{c}{0.325} &
  \multicolumn{1}{c}{0.591} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.044} &
  \multicolumn{1}{c}{0.325} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.044} &
  \multicolumn{1}{c}{0.339} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.045} &
  \multicolumn{1}{c}{0.344} &
  \multicolumn{1}{c}{0.551} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.049} &
  \multicolumn{1}{c}{0.349} &
  \multicolumn{1}{c}{0.576} \\ \midrule\midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{0.040}} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.610} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.344} &
  \multicolumn{1}{c}{0.601} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.339} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.050} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.046} &
  \multicolumn{1}{c}{\textbf{0.374}} &
  \multicolumn{1}{c}{\textbf{0.625}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.044} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.591} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.047} &
  \multicolumn{1}{c}{0.374} &
  \multicolumn{1}{c}{0.605} \\ \bottomrule
  \addlinespace
\end{tabular}%
 }
\end{table*}

\begin{table*}[hbt!]
\centering
\caption{\label{tab:TripletLoss-DataAugmentation} Normalized Average Rank (NAR) and Recall@K values for data augmentation experiments with Triplet Loss.}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{@{} l l l l l | l l l l l l @{}}
\toprule
\textbf{} &
  \textbf{} &
  \textbf{Image-Level} &
  \textbf{} &
   &
   &
  \textbf{Segment-Level} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
   \\ \midrule
\multicolumn{1}{c}{Resized Crop} &
  \multicolumn{1}{c}{Hor. Flip} &
  \multicolumn{1}{c}{Vert. Flip} &
  \multicolumn{1}{c}{Rotation} &
  \multicolumn{1}{c}{Color Jitter} &
  \multicolumn{1}{|c}{S. Color Change} &
  \multicolumn{1}{c}{S. Rotation} &
  \multicolumn{1}{c}{S. Removal} &
  \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
  \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
  \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
\multicolumn{8}{c}{\textit{Baseline}} &
  \multicolumn{1}{c}{0.102} &
  \multicolumn{1}{c}{0.310} &
  \multicolumn{1}{c}{0.536} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.053} &
  \multicolumn{1}{c}{0.339} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.052} &
  \multicolumn{1}{c}{0.349} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.052} &
  \multicolumn{1}{c}{0.364} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.051} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.054} &
  \multicolumn{1}{c}{0.320} &
  \multicolumn{1}{c}{0.546} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.053} &
  \multicolumn{1}{c}{0.344} &
  \multicolumn{1}{c}{0.591} \\ \midrule \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.369} &
  \multicolumn{1}{c}{0.601} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.052} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.052} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.050} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{0.046}} &
  \multicolumn{1}{c}{\textbf{0.374}} &
  \multicolumn{1}{c}{\textbf{0.640}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.571} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{0.046}} &
  \multicolumn{1}{c}{0.369} &
  \multicolumn{1}{c}{0.581} \\ \bottomrule
  \addlinespace
\end{tabular}
%
}
\end{table*}

==> ICPR2022 -- Logo Retrieval/logo_analysis.tex <==

\begin{table*}[ht]
    \centering
    \caption{\label{tab:RebuttalLogoAnalysis} Effect of text on logo retrieval performance. When used as queries, logos with text are more difficult to match to the logos in the dataset and the best and average ranks of similar logos are very low.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}lllllllll@{}}
        \toprule
        \multicolumn{1}{c|}{\textbf{Query}} &
        \multicolumn{1}{c}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/4-32.jpg}} &
        \multicolumn{1}{c|}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/10-32.jpg}} &
        \multicolumn{1}{c}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/12-30.jpg}} &
        \multicolumn{1}{c|}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/2-30.jpg}} &
        \multicolumn{1}{c}{\includegraphics[width=15mm, height=10mm]{Analysis Logos/10-4.jpg}} &
        \multicolumn{1}{c|}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/4-4.jpg}} &
        \multicolumn{1}{c}{\includegraphics[width=18mm, height=8mm]{Analysis Logos/11-26.jpg}} &
        \multicolumn{1}{c}{\includegraphics[width=10mm, height=10mm]{Analysis Logos/14-26.jpg}} \\ \midrule \midrule
        \multicolumn{1}{c|}{\textbf{Best Rank}} &
        \multicolumn{1}{c}{39k} &
        \multicolumn{1}{c|}{2} &
        \multicolumn{1}{c}{25} &
        \multicolumn{1}{c|}{5} &
        \multicolumn{1}{c}{97k} &
        \multicolumn{1}{c|}{1} &
        \multicolumn{1}{c}{159k} &
        \multicolumn{1}{c}{1} \\ \midrule \midrule
        \multicolumn{1}{c|}{\textbf{Average Rank}} &
        \multicolumn{1}{c}{253k} &
        \multicolumn{1}{c|}{2605} &
        \multicolumn{1}{c}{53k} &
        \multicolumn{1}{c|}{10k} &
        \multicolumn{1}{c}{239k} &
        \multicolumn{1}{c|}{25k} &
        \multicolumn{1}{c}{239k} &
        \multicolumn{1}{c}{1263} \\ 
         \bottomrule
        \addlinespace
        \end{tabular}
            }
\end{table*}

    
\begin{table}[ht]
\centering
\caption{\label{tab:LogoTypeAnalysis} Effect of text on logo retrieval performance using the 213 query logos in the METU Trademark Dataset.}
\begin{tabular}{@{}lll@{}}
    \toprule
    \multicolumn{1}{c}{\textbf{Logo Type}} &
    \multicolumn{1}{c}{\textbf{Number of Logos}} &
    \multicolumn{1}{c}{\textbf{NAR}} \\ \midrule \midrule
    \multicolumn{1}{c}{Logos w/o text} &
    \multicolumn{1}{c}{117} &
    \multicolumn{1}{c}{0.015} \\  \midrule
    \multicolumn{1}{c}{Logos w text} &
    \multicolumn{1}{c}{86} &
    \multicolumn{1}{c}{0.071} \\
     \bottomrule
    \addlinespace
    \end{tabular}
    \end{table}

==> ICPR2022 -- Logo Retrieval/sect_conclusion.tex <==
\section{Conclusion}

We introduced a novel data augmentation method based on image segments for training neural networks for logo retrieval. We performed segment-level augmentation by identifying segments in a logo and do transformations on selected segments. Experiments were conducted on the METU \cite{Kalkan} and LLD \cite{sage2017logodataset} datasets with ResNet \cite{ResNet} and ConvNeXt \cite{liu2022convnet} backbones and suggest significant improvements on two evaluation measures of ranking performance.  Moreover, we use metric learning and differentiable ranking with the proposed segment-augmentation method to demonstrate that our method can lead to a further boost in ranking performance. %In the future work, we will apply our method with effective proposed approaches to analyze the further improvement in retrieval performance. 

We note that our segment-level augmentation strategy generates similarities between logos that are rather simplistic: It is based on the assumption that two similar logos differ from each other in terms of certain segments having differences in color, orientation and presence. An important research direction is exploring more sophisticated augmentation strategies for introducing artificial similarities. However, our results suggest that even such a simplistic strategy can improve the retrieval performance significantly and therefore, our study can be considered as a first step towards developing better segment/part-level augmentation strategies.

==> ICPR2022 -- Logo Retrieval/sect_experiments.tex <==
\section{Experiments and Results}

We now evaluate the performance of the proposed segment-augmentation strategy and its use with Triplet Loss and Smooth-AP Loss. 

\subsection{Experimental and Implementation Details}

\subsubsection{Dataset}

We use the METU Dataset \cite{Kalkan}, which is one of the largest publicly available logo retrieval datasets. The dataset is composed of more than 900K authentic logos belonging to actual companies worldwide. Moreover, it includes query sets, i.e. similar logos, of varying difficulties, allowing logo retrieval researchers to benchmark their methods against other methods. We have used 411K training images, 413K test images, and 418 query images. %Description of the dataset is provided in Table \ref{tab:table-name}.

\begin{comment}
\begin{table}[htb]
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Aspect}                       & \textbf{Value}   \\ \midrule
Trademarks                            & 923,343          \\
Unique Register Firms                 & 409,675          \\
Unique Trademarks                     & 687,842          \\
Trademarks Containing Text Only       & 583,715          \\
Trademarks Containing Figure Only     & 19,214           \\
Trademarks Containing Figure and Text & 310,804          \\
Other Trademarks                      & 9,610            \\
Image Format                          & JPEG             \\
Max Resolution                        & 1800 $\times$ 1800 pixels \\
Min Resolution                        & 30 $\times$ 30 pixels     \\ \bottomrule
\addlinespace
\end{tabular}
\caption{\label{tab:table-name} Details of METU Dataset \cite{Kalkan}.}
\end{table}
\end{comment}

\subsubsection{Training and Implementation Details}

For every experiment that will be discussed, we use ImageNet \cite{ImageNet} pre-trained ResNet50 \cite{ResNet} as our backbone architecture which has a linear layer with 512 dimensions, rather than a final Softmax layer. We use the Adam optimizer with the hyper-parameters tuned as $10^{-7}$ for the learning rate and 256 for the batch size.

%As a result of the experiments, we observed that the ranking performance increased as the batch size increased. The best results were obtained when the batch size is set to 256. After various trials, learning rate is set to $10^{-7}$ to achieve the best ranking performance. 

\subsubsection{Evaluation Measures}

Following the earlier studies \cite{Kalkan,Tursun2019}, we use  {Normalized Average Rank} (NAR) and {Recall@K} for quantifying the performance of the methods. NAR is calculated as:
%
\begin{equation}
  {NAR = \frac{1}{N\times N_{rel}} \left(\sum_{i=1}^{N_{rel}} R_i - \frac{N_{rel}(N_{rel}+ 1)}{2} \right)},
\end{equation}
%
where $N_{rel}$ is the number of similar images for a particular query image; $N$ is the size of the image set;  and $R_i$ is the rank of the $i^{th}$ similar image. NAR lies in the range $[0,1]$, where $0$ denotes the perfect score, and $1$ the worst. Recall@K (R@K) is recall for top-K similar logos.

\begin{table}[hbt!]
\centering
\caption{\label{tab:RankingLossesTable} The effect of using Triplet Loss and Smooth-AP Loss for logo retrieval.  Neither image-level nor segment-level augmentation is used for any method in this table.}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Method}  & \textbf{NAR} $\downarrow$   & \textbf{Recall@1} $\uparrow$   & \textbf{Recall@8} $\uparrow$    \\ \midrule
Baseline       & 0.102          & 0.310          & 0.536          \\ \midrule
Triplet Loss   & 0.053          & \textbf{0.344} & \textbf{0.586} \\ \midrule
Smooth-AP Loss & \textbf{0.046} & 0.339          & 0.581          \\ \bottomrule
\addlinespace
\end{tabular}
\end{table}

\subsection{Experiment 1: Effect of Ranking Losses}

Before analyzing the effect of segment-level augmentation, in this section, we first provide a stand-alone analysis to illustrate the effect of the ranking losses. We compare Triplet Loss and Smooth-AP Loss with a baseline that compares features extracted with the pre-trained Resnet50 backbone using Cosine Similarity. For this analysis, no image-level or segment-level augmentations are used, except for the Random Resized Crop to fit the images to the expected resolution of the network, i.e.  $224 \times 224$. 

The results in Table \ref{tab:RankingLossesTable} suggest that both loss adaptations provide a significant performance improvement in both NAR and Recall measures and Smooth-AP adaptation achieves the best performance.  Applying Cosine Similarity on off-the-shelf ResNet50 features shows adequate results in no-text logo instances, however, it performs worse on logos with text (see Appendix E). 

It is evident that the improvement in Recall is not as visible as NAR. This difference states that the adapted loss functions highly affect the overall rankings of the similar known instances. However, these effects are not completely reflected by the Recall because of the selected K$=8$ value.  

\begin{table}[ht]
\centering
\caption{\label{tab:BestAugmentationResults} The effect of image-level (H. Flip, V. Flip) and segment-level augmentation. Only the best augmentation strategies are reported. See Section \ref{sect:ablation} for an ablation analysis.}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Method}  & \textbf{NAR} $\downarrow$   & \textbf{Recall@1} $\uparrow$   & \textbf{Recall@8} $\uparrow$    \\ \midrule

Baseline\\
(No augmentation) & 0.102          & 0.310          & 0.536          \\ \midrule\midrule
Triplet Loss\\
(No augmentation)& 0.053 & 0.344 & 0.586 \\ \midrule
Triplet Loss\\
(Image-level aug.) & 0.051          & 0.354 & 0.596 \\ \midrule
Triplet Loss\\
(S. Color, S. Removal) & 0.046          & \textbf{0.374} & \textbf{0.640} \\ \midrule\midrule
Smooth-AP Loss\\
(No augmentation) & 0.046          & 0.339 & 0.581 \\ \midrule
Smooth-AP Loss\\
(Image-level aug.) & 0.044          & 0.339 & 0.596 \\ \midrule
Smooth-AP Loss \\
(S. Color)  & \textbf{0.040} & 0.354          & 0.610          \\ \bottomrule
\addlinespace
\end{tabular}
\end{table}

\begin{table}[hbt!]
\centering
\caption{\label{tab:SOTATable} Normalized Average Rank (NAR) values for previous state-of-the-art results on the METU dataset. The results are not comparable as the methods differ in their backbones, training datasets, or training regime. For some methods, these details are not even reported. See the text for details.}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Method}  & \textbf{NAR} $\downarrow$\\ \midrule
Hand-crafted Features (Feng \emph{et al.} \cite{Feng}) & 0.083 \\ \midrule
Hand-crafted Features (Tursun \emph{et al.} \cite{Kalkan})  & 0.062 \\ \midrule
Off-the-shelf Deep Features (Tursun \emph{et al.} \cite{TursunandKalkan})  & 0.086 \\ \midrule
Transfer Learning (Perez \emph{et al.} \cite{Perez})   & 0.047  \\ \midrule
Component-based attention (SPoC \cite{SPOC}, \cite{Tursun2019}) & 0.120  \\ \midrule
Component-based attention (CRoW \cite{CRoW}, \cite{Tursun2019}) & 0.140  \\ \midrule
Component-based attention (R-MAC \cite{MAC}, \cite{Tursun2019}) & 0.072  \\ \midrule
Component-based attention (MAC \cite{MAC} \cite{Tursun2019}) & 0.120  \\ \midrule
Component-based attention (Jimenez \cite{Jimenez},\cite{Tursun2019}) & 0.093  \\ \midrule
Component-based attention (CAM MAC \cite{Tursun2019}) & 0.064  \\ \midrule
Component-based attention (ATR MAC \cite{Tursun2019}) & 0.056  \\ \midrule
Component-based attention (ATR R-MAC \cite{Tursun2019}) & 0.063  \\ \midrule
Component-based attention (ATR CAM MAC \cite{Tursun2019}) & 0.040 \\ \midrule
MR-R-MAC w/UAR (Tursun \emph{et al.} \cite{Tursun2022}) & {0.028} \\ \midrule
Segment-Augm. (Color Change) w Smooth-AP (Ours)   & {0.040}  \\
\bottomrule
\addlinespace
\end{tabular}
\end{table}


\subsection{Experiment 2: Effect of Segment Augmentation}

We now compare our segment-based augmentation methods with the conventional image-level augmentation techniques on the METU dataset \cite{Kalkan}. In every experiment, we resize the images with Random Resized Crop to fit them to the expected resolution of the network, i.e. 224$\times$224. For both segment-based and image-level augmentation, the same number of images are augmented and the probability $p=0.5$ is used for selecting a certain transformation.
 
We have provided a comparison between the best resulting methods for both image-level and segment-level augmentation methods in Table \ref{tab:BestAugmentationResults}. We see that image-level augmentation can improve ranking performance. However, the results suggest that segment-level augmentation provides a significantly better gain both in terms of NAR and R@K measures. Detailed comparison between image-level and segment-level methods is provided in ablation study.





\subsection{Experiment 3: Comparison with State of the Art}

We compare our method and the state-of-the-art methods on the METU dataset \cite{Kalkan}. It is important to note that a fair comparison between the methods is not possible because they differ in their backbones, training datasets or dataset splits, or training time. For some papers, even those details are missing; e.g. for \cite{Tursun2022}, which reports the best NAR performance. Therefore, we list the results in Table \ref{tab:SOTATable}, and refrain from drawing conclusions.

\begin{table}[ht]
    \centering
    \caption{\label{tab:ProbabilityTable} The effect of probability $p$ for augmenting a selected segment, with Smooth-AP Loss.}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        \multicolumn{1}{c}{Color C.} &
        \multicolumn{1}{c}{Rotation} &
        \multicolumn{1}{c}{Removal} &
        \multicolumn{1}{c}{\textbf{$p$}} &
        \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
        \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
        \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule \midrule
        \multicolumn{3}{c}{\textit{Baseline}} &
        \multicolumn{1}{c}{0} &
        \multicolumn{1}{c}{0.046} &
        \multicolumn{1}{c}{0.339} &
        \multicolumn{1}{c}{0.581}  \\ \midrule \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{\textbf{0.040}} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{\textbf{0.610}}  \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.043} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{0.601}  \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{0.325} &
        \multicolumn{1}{c}{0.566} \\ \midrule \midrule
         \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.601}  \\ \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{\textbf{0.369}} &
        \multicolumn{1}{c}{0.591}  \\ \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.060} &
        \multicolumn{1}{c}{0.330} &
        \multicolumn{1}{c}{0.556} \\ \midrule \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.339} &
        \multicolumn{1}{c}{0.596} \\ \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.571} \\  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.591} \\
         \bottomrule
        \addlinespace
        \end{tabular}
    \end{table}

% \begin{table}[ht]
%     \centering
%     \caption{\label{tab:NTable} The effect of the number of segments $n$ selected for augmentation, with Smooth-AP Loss. $L$ denotes the total number of segments in a logo.}
%     \scriptsize
%         \begin{tabular}{@{}lllllll@{}}
%         \toprule
%         \multicolumn{1}{c}{Color} &
%         \multicolumn{1}{c}{Rotation} &
%         \multicolumn{1}{c}{Removal} &
%         \multicolumn{1}{c}{\textbf{$n$}} &
%         \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
%         \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
%         \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule \midrule
%         \multicolumn{3}{c}{\textit{Baseline}} &
%         \multicolumn{1}{c}{0} &
%         \multicolumn{1}{c}{0.046} &
%         \multicolumn{1}{c}{0.339} &
%         \multicolumn{1}{c}{0.581}  \\ \midrule \midrule
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{$\frac{L}{3}$} &
%         \multicolumn{1}{c}{\textbf{0.040}} &
%         \multicolumn{1}{c}{0.354} &
%         \multicolumn{1}{c}{\textbf{0.610}}  \\ \midrule
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{$\frac{L}{2}$} &
%         \multicolumn{1}{c}{0.043} &
%         \multicolumn{1}{c}{0.354} &
%         \multicolumn{1}{c}{0.601} &  \midrule
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{L} &
%         \multicolumn{1}{c}{0.049} &
%         \multicolumn{1}{c}{0.325} &
%         \multicolumn{1}{c}{0.566} &  \midrule \midrule
%          \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{1} &
%         \multicolumn{1}{c}{0.048} &
%         \multicolumn{1}{c}{0.344} &
%         \multicolumn{1}{c}{0.601} &  \midrule
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{$\frac{L}{2}$} &
%         \multicolumn{1}{c}{0.049} &
%         \multicolumn{1}{c}{\textbf{0.369}} &
%         \multicolumn{1}{c}{0.591}  \\ \midrule
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{L} &
%         \multicolumn{1}{c}{0.060} &
%         \multicolumn{1}{c}{0.330} &
%         \multicolumn{1}{c}{0.556} \\ \midrule \midrule
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{1} &
%         \multicolumn{1}{c}{0.048} &
%         \multicolumn{1}{c}{0.339} &
%         \multicolumn{1}{c}{0.596} \\ \midrule
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{2} &
%         \multicolumn{1}{c}{0.047} &
%         \multicolumn{1}{c}{0.344} &
%         \multicolumn{1}{c}{0.571} \\  \midrule
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\checkmark} &
%         \multicolumn{1}{c}{$\frac{L}{2}$} &
%         \multicolumn{1}{c}{0.047} &
%         \multicolumn{1}{c}{0.344} &
%         \multicolumn{1}{c}{0.591} &
%          \bottomrule
%         \addlinespace
%         \end{tabular}
% \end{table}

\input{buyuk_tablo}

\subsection{Experiment 4: Ablation Study}
\label{sect:ablation}

\subsubsection{Choice of Hyper-Parameters}

Our segment-level augmentation has two hyper-parameters: The number of segments, $n$, selected for augmentation, and the probability, $p$, of applying a selected augmentation. Table \ref{tab:ProbabilityTable} shows that the best performance is obtained with $p$ as 0.5. A similar analysis for $n$ (with values 1, 2, $L/3$ and $L/2$ where $L$ is the number of segments in a logo) provided the best performance for $n$ as $L/3$. 

\subsubsection{Effects of Individual Augmentation Methods}

Tables \ref{tab:SmoothAP-DataAugmentation} (Smooth-AP Loss) and \ref{tab:TripletLoss-DataAugmentation} (Triplet Loss) list the effects of both image-level and segment-level augmentation. The tables show that, among the segment-level augmentation methods, (Segment) `Color Change' outperforms the others for both loss functions. With Triplet Loss adaptation, (Segment) `Removal' and `Rotation' provide slightly better NAR values than the baseline. Another point worth mentioning is that combining (Segment) `Rotation' or `Removal' degrades the NAR performance measure whereas the combination of (Segment) `Removal' and `Color Change' yields the best result at $Recall@8$.

\subsubsection{Experiments with a Different Backbone}

Section A in the Appendix provides an analysis using ConvNeXt \cite{liu2022convnet}, a recent, fast and strong backbone competing with transformer-based architectures. Our results without any hyper-parameter tuning are comparable to the baseline or better than the baseline with the R@8 measure.

\subsubsection{Experiments with a Different Dataset}

Section B in the Appendix reports results on the LLD dataset \cite{sage2017logodataset} that confirm our analysis on the METU dataset: We observe that segment-level augmentation provides significant gains for all measures.

% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/visual_results.pdf}
%     \caption{Sample visual results for the baseline, Triplet Loss (segment color change and removal) and Smooth-AP Loss (segment color change) with their best settings.}
%     \label{fig:visual_results}
% \end{figure}


\subsection{Experiment 5: Visual Results}

Section F in the Appendix provides sample retrieval results for several query logos for the baseline as well the adaptations of Triplet Loss and Smooth-AP Loss with our segment-level augmentation methods. The visual results also confirm that segment augmentation with our Smooth-AP adaptation performs best.



==> ICPR2022 -- Logo Retrieval/sect_introduction.tex <==
\section{Introduction}
% no \IEEEPARstart
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)

\begin{figure}[hbt!]
\centering
\includegraphics[width=0.99\columnwidth]{Figures/teaser.pdf}
\caption{(a) Conventional data augmentation approaches apply transformations at the image level. (b) We propose segment-level augmentation as a more suitable approach for problems like logo retrieval.
\label{fig_teaser}}
\end{figure}


With the rapid increase in companies founded worldwide and the fierce competition among them globally, the identification of companies with their logos has become more pronounced, and it has become more paramount to check similarities between logos to prevent trademark infringements. Checking trademark infringements is generally performed manually by experts, which can be sub-optimal due to human-caused errors and time-consuming as it takes days to make a decision. Therefore, automatically identifying similar logos using content-based image processing techniques is crucial.

For a query logo, identifying the similar ones in a database of logos is a content-based image retrieval problem. With the rise in deep learning, there have been many studies that have used deep learning for logo retrieval problem \cite{Tursun2019, Feng, unsupervisedattention, Tursun2022, Perez}. Existing approaches generally rely on extracting features of logos and ranking them according to a suitable distance metric \cite{TursunandKalkan, Tursun2019, Perez}.

Logo retrieval is a challenging problem especially for two main reasons: (i) Similarity between logos is highly subjective, and similarity can occur at different levels, e.g., texture, color, segments and their combination etc. (ii) The amount of known similar logos is limited. We hypothesize that this has limited the use of more modern deep learning solutions, e.g. metric learning, contrastive learning, differentiable ranking, as they require tremendous amount of positive pairs (similar logos) as well as negative pairs (dissimilar logos) for training deep networks.

In this paper, we address these challenges by (i) proposing a segment-level augmentation to produce artificially similar logos and (ii) using metric learning (Triplet Loss \cite{weinberger2009distance}) and differentiable ranking (Smooth Average Precision (AP) Loss \cite{Brown2020eccv}) as a proof of concept that, with our novel segment-augmentation method, such data hungry techniques can be trained better. 

\textit{Main Contributions.} Our contributions are as follows:
\begin{itemize}
    \item We propose a segment-level augmentation for producing artificial similarities between logos. To the best of our knowledge, ours is the first to introduce segment-level augmentation into deep learning. Unlike image-level augmentation methods that transform the overall image, we identify segments in a logo and make transformations at the segment level. Our results suggest that this is more suitable than image-level augmentation for logo retrieval.
    
    \item To showcase the use of such a tool to generate artificially similar logos, we use data-hungry deep learning methods, namely, Triplet Loss \cite{weinberger2009distance} and Smooth-AP Loss \cite{Brown2020eccv}, to show that our novel segment-augmentation method can indeed yield better retrieval performance. To the best of our knowledge, ours is the first to use such methods for logo retrieval.
\end{itemize}


%According to literature, a logo is a graphic representation or symbol of a company name, trademark, abbreviation, often uniquely designed for ready recognition. Similarly, a trademark can be defined as a name, symbol, figure, letter, word, or mark adopted and used by a manufacturer or merchant to designate specific goods and distinguish them from those manufactured or sold by others. According to World Intellectual Property Organization \cite{WIPO} , 3 million trademark registrations exist worldwide, and trademark applications have kept increasing at a rate of 6-8{\%} in recent years. Trademark infringements have become an essential yet challenging problem due to an ever-increasing trademark application trend \cite{WIPO}. Several methods include image retrieval with neural networks to detect trademark infringements. The main idea is to retrieve the most similar trademarks according to the query trademark. Hence, it is a ranking problem. However, these methods have two main challenges:

%\begin{itemize}
%    \item \textbf{Similarity Aspect} - Unlike object similarity, trademark similarity mostly depends on the visual similarity aspect. Semantically unfamiliar two logos can be familiar in terms of visual similarity. Currently, available image retrieval techniques focus on object-related similarity. Since trademarks are elementary images according to most images - they have less features compared to others-, object-related techniques are more prone to unsatisfactory results.
%    \item \textbf{Lack of Dataset} - There is not enough data publicly for the analysis of the methods. METU LOGO Dataset \cite{Kalkan} can be an excellent solution for this problem; however, sufficient data does not have a significant impact without an efficient method.
%\end{itemize}


%\begin{figure}[!h]
%\centering
%\includegraphics[width=2.5in]{Figures/similarity.jpg}
%\caption{Sample trademark similarities.}
%\label{fig_similarity}
%\end{figure}

%The similarity definition of the trademark retrieval problem has multiple aspects rather than one, causing a challenge not encountered in common retrieval problems. The lack of known similar trademark instances causes a challenge to train this similarity definition to the model. 
%Data augmentation is a widely used technique to increase the diversity of samples in a dataset. These methods mostly lead to increased overall performance in both image classification and retrieval problems, especially when the dataset is unbalanced. Since trademarks have less features compared to others, region-based similarities have a crucial effect on the trademark similarity. Hence, to increase the diversity of these known similar instances, we introduce a novel non-trivial data augmentation method based on the trademark segments to improve retrieval performance. We observed that our region-based augmentation leads us to obtain more complex similarities, resulting in noticeable performance gain compared to well-known augmentation methods.


%Additionally, we further improve the retrieval performance by using ranking-based methods that optimize the standard retrieval metric, Average Precision. Smooth-AP \cite{Brown2020eccv} is a novel that obtains state-of-the-art results in benchmark retrieval tasks. Its expected contribution is a differentiable approximation of the average precision to improve the retrieval performance. However, since it is impossible to separate trademarks into classes according to their similarity, Smooth-AP \cite{Brown2020eccv} can not be directly applied to our trademark retrieval problem. Moreover, we have adapted the Smooth-AP method to conform to the class-independent definition of the trademark retrieval problem. We conducted experiments of these proposed methods with the large scaled METU Trademark Dataset \cite{Kalkan} and obtained significant results. 


==> ICPR2022 -- Logo Retrieval/sect_method.tex <==
\section{Method}

In this section, after providing a definition for logo retrieval, we present our novel segment-based augmentation method and how we use it with deep metric learning and differentiable ranking approaches. % first explains the mini-batch sampling for the training process. Next, the different segment-based augmentation methods, namely, Segment Color Change, Segment Rotation and Segment Removal, are introduced. Finally, the adaptations of the ranking-based loss functions are discussed.

\begin{wrapfigure}{r}{0.45\columnwidth}
\centering
\includegraphics[width=0.45\columnwidth]{Figures/sample_augmentations.pdf}
\caption{Examples for our segment-level augmentation.}
\label{fig_augmentation}
\end{wrapfigure}

\subsection{Problem Definition}

Given an input query logo $I_q$, logo retrieval aims to rank all logos in a retrieval set $\Omega$ = ${I_i}$, $i=\{0,1,..., N\}$, based on their similarity to the query $I_q$. To be able to evaluate retrieval performance and to train a deep network that relies on known similarities, we require for each $I_q$ to have a set of positive (similar) logos, $\Omega^+(I_q)$, and a set of negative (dissimilar) logos, $\Omega^-(I_q)$. Note that logo retrieval defined as such does not have the notion of classes of a classification setting.


\subsection{Segment-level Augmentation for Logo Retrieval}

We perform segment-level augmentation by following these steps: (i) Logo segmentation, (ii) segment selection, and (iii) segment transformation. See Figure \ref{fig_augmentation} for some samples.
\begin{wrapfigure}{r}{0.45\columnwidth}
  \centering
  \vspace*{-4cm}
    \includegraphics[width=0.45\columnwidth]{Figures/segmentation.pdf}
    \caption{Sample segmentation results. Each segment is represented with different color.}
    \label{fig_segmentation}
\end{wrapfigure}

%We assume that segment-level augmentation does not change the similarity between two logos; i.e., if an instance is a similar instance, it’s augmented instance is still a similar instance. During training, we only apply our method to the instances of the $\omega_+$ in each mini batch. For each instance of $\omega_+$, the probability of applying selected segmentation augmentation is $p$.

\subsubsection{Logo Segmentation}

There are many sophisticated segmentation approaches available in the literature. Since logo images have relatively simpler regions compared to images, we observed that a simple and computationally-cheap approach using standard connected-component labeling is sufficient for extracting logo segments. See Figure \ref{fig_segmentation} for some samples, and Supp. Mat. Section S4 for more samples and a discussion on the effect of segmentation quality.


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.4\columnwidth]{Figures/segmentation.pdf}
%     \caption{Sample segmentation results. Each segment is represented with different color.}
%     \label{fig_segmentation}
% \end{figure}

\subsubsection{Segment Selection}

The next step is to select $n$ random segments to apply  transformations on them. Segment selection is a process that should be evaluated carefully since the number of segments or the area for each segment is not the same for each logo. Simplicity of logo instances also affects the number of available components and many logo instances have less than five components. Therefore, the choice of $n$ can have drastic effects especially when the number of components in a logo is small, especially for the `segment removal' transformation. For this reason, `segment removal' is not applied to a segment with the largest area, and $n$ is chosen to be small values. We present an ablation study to evaluate the effect of $n$ on model performance for the introduced augmentation strategies. For the same reason, the background component is removed from available segments for augmentation.

\subsubsection{Segment Transformation}

For each selected segment $S$, the following are performed with probability $p$:
\begin{itemize}
    \item `(Segment) Color change': Every pixel in $S$ is assigned to a randomly selected color. 
    \item `Segment removal': Pixel values in $S$ are set to the same value of the background component.
    \item `Segment rotation': We first select a segment and create a mask for the segment. The mask image and the corresponding segment pixels are rotated with a random angle in [-90, 90]. Then, the rotated segment is combined with the other segments. See also Figure \ref{fig_segment_rotation} for an example.
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/rotation_steps.pdf}
    \caption{The steps of rotating a segment.}
    \label{fig_segment_rotation}
\end{figure}

See Figure \ref{fig_augmentation} for some sample augmentations.

% \begin{figure}[!t]
% \centering
% \includegraphics[height=2in]{Figures/sample_augmentations.pdf}
% \caption{Examples for our segment-level augmentation.}
% \label{fig_augmentation}
% \end{figure}



\subsection{Adapting Ranking Losses for Logo Retrieval}

\subsubsection{Mini-batch Sampling for Training}
\label{sect:minibatch}
%Each mini-batch is constructed in a way that, for each minibatch, there are a specific amount of (3, 4, or 5 for different experiments) instances of a known labeled class. A known labeled class is a class that has instances of similar images for some query image. The remaining batch is constructed from the instances that do not have any similarity with other instances. In every mini-batch, we select the known class randomly. For each mini-batch, there are two classes; one is the known labeled class, we label them as "1" and the other class "0", instances of gallery dataset.
For training the deep networks, we construct the batches as follows, similar to but different from \cite{Brown2020eccv} as we do not have classes: Each mini-batch $B$ with size $|B|$ is constructed with two sub-sets: the similar set $B^{+}$ and the dissimilar set $B^{-}$. The similar logo set $B^{+}$ consists of logos that are known to be similar to each other (this information is available in the dataset \cite{Kalkan}; logos with known similarities are provided as the ``query set''), and $B^{-}$ contains logos that are dissimilar to the logos in $B^{+}$ (to be specific, logos other than the query set of the dataset are randomly sampled for $B^{-}$). The size of $B^{+}$ is set to $4$, and that of $B^{-}$ is $|B|-4$. For training the network, every $I \in B^{+}$ has label as ``1'' and $I \in B^{-}$ has label ``0''.




\subsubsection{Smooth-AP Adaptation}

Smooth-AP \cite{Brown2020eccv} is a ranking-based differentiable loss function, approximating AP. The main aspect of this approximation is to replace discrete counting operation (the indicator function) in the non-differentiable AP with a Sigmoid function. Brown et al. \cite{Brown2020eccv} applied their study to standard retrieval benchmarks such as Stanford Online Products \cite{song2016deep}, VGGFace2 \cite{DBLP:journals/corr/abs-1710-08092} and VehicleID \cite{liu2016deep}. However, the logo retrieval problem requires a dataset with a different structure as there is no notion of classes as in the Stanford Online Products \cite{song2016deep}, VGGFace2 \cite{DBLP:journals/corr/abs-1710-08092} and VehicleID \cite{liu2016deep} datasets. Hence, Smooth-AP cannot be applied directly to our problem.

The first adaptation is about the structure of the mini-batch sampling. In Smooth-AP, Brown et al. explain their sampling as they have \textit{``formed each mini-batch by randomly sampling classes such that each represented class has P samples per class''} \cite{Brown2020eccv}. Standard retrieval benchmarks have a notion of classes and are assumed to have sufficient instances per class to distribute among the mini-batches; however, there are not enough instances for known similarity ``classes'' in logo retrieval. This difference requires an adaption in both sampling and calculation of the loss. Smooth-AP Loss is calculated as follows \cite{Brown2020eccv}:
%
\begin{equation}
{\mathcal{L}_{AP}} = {\frac{1}{C}} {\sum_{k=1}^{C} (1-\tilde{AP}_{k})} ,
\end{equation}
%
where $C$ is the number of \textit{classes} and $\tilde{AP}_k$ is the smoothed AP calculated for each class in the mini-batch with their Sigmoid-based smoothing method.

Our mini-batch sampling (Section \ref{sect:minibatch}) causes a natural contradiction because our batches only contain two classes: ``similar'' and ``dissimilar''; therewith the ``dissimilar'' class should not be included in the calculation of the loss. Dissimilar class instances have the same label (``0''), but that does not mean they have the same class; they are just not similar to the similar logo set $B^+$ in the mini-batch.
Hence, the ranking among $B^-$ does not matter in our case. This difference in the batch construction and the notion of classes lead to our second adaptation. In this adaptation, the only calculated AP approximation belongs to the known ``similar'' class (logos in $B^+$). Therefore, the loss calculation becomes:
%
\begin{equation}
    \mathcal{L}^+_{AP} = 1-{\tilde{AP}_+},
\end{equation}
%
where $\tilde{AP}$ is calculated (approximated) in the same way as in the original paper \cite{Brown2020eccv}. 

\subsubsection{Triplet Loss Adaptation}

Triplet Loss \cite{weinberger2009distance} is a well-known loss function used in many computer vision problems. Triplet Loss is  differentiable, but, unlike Smooth-AP Loss \cite{Brown2020eccv}, rather than optimizing ranking, it optimizes the distances between positive pairs and negative pairs of instances. In this paper, for each mini-batch, triplets consist of one ``anchor" instance, one positive instance, and one negative instance. For the same reasons discussed in Smooth-AP Loss \cite{Brown2020eccv}, only the instances of known similarity classes can be used as the anchor instance. Optimizing the distances between dissimilar logo instances is not sensible because, as discussed in the previous section, instances of the dissimilar logos do not have any known similarity between them. Thus, triplet loss calculation is limited to the triplets that contain known similar instances as the ``anchor'' instance.

==> ICPR2022 -- Logo Retrieval/sect_rebuttal.tex <==



\section*{Authors' Response}

We thank all the reviewers for their valuable feedback. To summarize: The reviewers found our paper \textit{``well-motivated''} (\Rfour, \Rseven), \textit{``well-organized''} (\Rseven), \textit{``well-written''} (\Reight), containing \textit{``valuable ideas''} (\Rfour), and \textit{``interesting''} (\Reight) and noted that \textit{``experimental results demonstrate the effectiveness of the proposed strategy"} (\Rseven). The reviewers had concerns about the novelty of the ideas as well as the significance of the results. Moreover, they requested more analysis and a discussion of the limitations. 

We've addressed all reviewer comments and the quality of our paper improved significantly. To be specific, in addition to updating the text to clarify ambiguous points, we've conducted new experiments and we report positive results on another dataset ({LLD - Large Logo Dataset} \cite{sage2017logodataset} -- see item A3), with a more recent, stronger and fast backbone ({ConvNeXt} architecture \cite{liu2022convnet} -- see item {C1}), and provide a running-time analysis (C5), an analysis of the effect of text (C2), visual results (A2\&C6) and more discussion. In the following, we only summarize our changes and respond to the comments provided by the reviewers. Due to space limitations, the new results are provided in the supplementary material, with pointers placed in the main text.

\subsection{Common Concerns}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{A1. Simplicity of the Contribution.} 
\Rsix: \textit{``[t]he contribution and novelty of this paper are limited since the authors propose a standard application of well-known methods according to a classic algorithmic scheme (the proposed techniques are simple and already proposed in the literature)"}. \Reight: \textit{``idea of the proposed "segment level" augmentation appears more as an engineering, rather than a scientific contribution"}.

\Authors: We respectfully disagree with the reviewers on the requirement that a paper's methodology should be sophisticated or non-engineered: (i) [Computer] Science makes progress by putting together existing tools and methods in novel ways for solving problems, generally improving some performance measures while doing so. In our case, we do use existing tools (segmentation, augmentation) but propose a novel idea for combining them for solving an existing problem with a significantly better performance. (ii) An `engineering' approach can be scientific if the engineered solution is novel. (iii) There exist similar papers at top conferences (``Copy-paste networks...",  ICCV2017 \cite{lee2019copy} ; ``Cut, paste and learn...", ICCV2019 \cite{dwibedi2017cut}; ``Simple copy-paste ...", CVPR2021 \cite{ghiasi2021simple}) that propose ``simple'' and ``engineered'' augmentation methods or analyze them. Such papers are scientific contributions as they contribute to the progress of [Computer] Science by bringing together existing tools in new ways or by analyzing what's not been known before. We strongly believe that our paper is similar, its contributions are scientific and our novel idea deserves to be seen by the community. Moreover, our novel way of performing \& analyzing segment-level augmentation has strong potential for inspiring more granular augmentation strategies than what's generally used in the literature (see also E2 \& Supp. Mat. Section S8-C).

\noindent\textbf{A2. Quality and Explanation of segmentation.}

\textbf{\Rfour}: \textit{``...quantitative results and performance of segmentation quality are not given"}. \textbf{\Rseven}: \textit{... segmentation errors, limitations and errors should be discussed.}

\Authors: We thank the reviewers for highlighting this important point. Logos are simplistic images composed of regions that are generally homogeneous in color. Therefore, an off-the-shelf simple segmentation algorithm works well for most logos (see Supp. Mat. Section S4 for some examples). Logo segmentation can produce spurious segments especially on regions which have strong color gradients. However, such infrequent cases are not a problem for us because segments corresponding to over-segmentation or under-segmentation do function as segment-level augmentation and this is still useful for training. We provide a discussion about this in  Supp. Mat. Section S4.

%The reviewers raise an important point, and we were unable to analyze this in the paper due to space limitations. As the logo datasets do not have segment We note that \renkli{...} Moreover, even when the segmentation methods produces faulty segments, such faulty (broken) segments do function as sub-segment level augmentation and this is not necessarily a negative problem for training. 

\noindent\textbf{A3. Other Datasets}

\textbf{\Rfour}: \textit{``I encourage the authors to point out the performance of their method on more benchmark datasets."}

\textbf{\Rsix}: \textit{``... Please conduct more experiments on other recent datasets."}

\Authors: With this revision, we've performed experiments with the {LLD - Large Logo Dataset} {\cite{sage2017logodataset}}. Our results (Supp. Mat. Section S2) confirm that the performing segment-level augmentation is a working strategy for learning better representations for trademark similarity. These results are obtained without any hyper-parameter tuning and we anticipate the gap to widen if they are tuned.

\input{LLD_table}
\subsection{Specific Concerns of \Rfour}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{B1 - \Rfour}:  \textit{``contributions of the paper are not clearly stated, so the novelty remains somewhat questionable."}

\Authors: The last two paragraphs of Introduction state our contributions as follows (truncated to save space): 

``\textit{Main Contributions.} Our contributions are as follows:
\begin{itemize}
    \item We propose a segment-level augmentation for producing artificial similarities between logos. To the best of our knowledge, ours is the first to introduce segment-level augmentation in deep learning. [...]
    
    \item To showcase the use of such a tool to generate artificially similar logos, we use data-hungry deep learning methods, namely, Triplet Loss \cite{weinberger2009distance} and Smooth AP \cite{Brown2020eccv}, [...]"
\end{itemize}

\noindent\textbf{B2 - \Rfour}: \textit{``...table I and table II are not evident in order to demonstrate the performance. What are the chosen hyperparameters?"}

\Authors: In Table I, we see the effect of applying ranking/comparison-based losses for logo retrieval. We see that both Triplet Loss and Smooth-AP Loss do significantly improve over the baseline. Although these results are new for logo retrieval, the methods are not novel for our paper. In Table II, we show that applying image-level augmentation improves logo retrieval performance; though we obtain better gain with our proposed way of performing segment-level augmentation. The hyper-parameters are provided in detail in Section IV.A.2.

\subsection{Specific Concerns of \Rsix}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{C1 - \Rsix}: \textit{``...the authors should compare their contribution with recent deep networks."}
\input{ConvNext_table}
\Authors: We now compare our method with a very recent CNN architecture, namely, ConvNeXt \cite{liu2022convnet}. The new results in Supp. Mat. Section S1 confirm our hypothesis that segment-level augmentation performs on par or improves logo retrieval performance. Our ongoing experiments with ResNext, which could not be completed because ResNext is slower than ResNet or ConvNeXt, also promise significant gain in favor of using segment-level augmentation (results will be included in the camera-ready version).

\noindent\textbf{C2 - \Rsix}: \textit{``...justify why ResNet performs worse on logos having text content in IV-B Experiment 1. ... give qualitative and quantitative performance analysis of this observation"}

\Authors: We now provide both qualitative \& quantitative results on this in Supp. Mat. Section S5, and provide a discussion.

\noindent\textbf{C3 - \Rsix}: \textit{``...why certain transformations in the data augmentation step are more performant when applying Triplet Loss, while other are better when using Smooth AP."}.

\Authors: This is an important point and we now provide a discussion on this in Supp. Mat. Section S8. To provide a summary here: Smooth AP and Triplet Loss incur different inductive ranking biases and this leads to different overall behaviors for the methods.

\noindent\textbf{C4 - \Rsix}: \textit{``...best value of p depends on the type of used transformation and the computed performance evaluation metric."}.

\Authors: The reviewer is right about this point. However, different augmentations incur different biases and it is not surprising that they contribute to performance differently and with different selection probabilities. We now provide a discussion about this in Supp. Mat. Section S8.

\noindent\textbf{C5 - \Rsix}: \textit{``...discussion on the complexity (e.g. training time and retrieval response) is missing."}

\Authors: We now provide a running-time analysis in Supp. Mat. Section S7.

\noindent\textbf{C6 - \Rsix}: \textit{``The authors should present an error analysis to find the reasons behind the incurred errors by analyzing correlations between the different scenarios."}

\Authors: We now provide more qualitative analysis in Supp. Mat. Sections S4 and S6 on failure cases as well and provide a discussion for potential reasons.

\noindent\textbf{C7 - \Rsix:} \textit{``The Triplet Loss function requires preparing a database done by triplets of images, limiting its application to the existing publicly available datasets."}

\Authors: Taking samples from a class as anchors \& positive samples, and samples from other classes as negative samples, applying Triplet Loss is actually very straightforward and can be applied to any classification or retrieval problem. This can be easily done on the run while sampling a batch without preparing a separate dataset.

\subsection{Specific Concerns of \Rseven}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{D1 - \Rseven}: \textit{"...Please further discuss the performance of triplet loss and smooth AP loss in Table \ref{tab:RankingLossesTable}}

\Authors: We now provide a discussion on this in Supp. Mat. Section S6. To provide a summary here: Smooth AP and Triplet Loss incur different inductive ranking biases and this leads to different overall behaviors for the methods.

\subsection{Specific Concerns of \Reight}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{E1 - \Reight:} ``\textit{The variety of image-level augmentation techniques, which were used for comparison, is insufficient and the selected techniques themselves are trivial. To improve the impact of that contribution a better comparison with other techniques should be performed. For instance, the are public implementations [1,2]."}

\Authors: We now compare with three more commonly-used image-level augmentation methods (namely, {Cutout, Elastic Transform and Channel Shuffle}) from the library  {\cite{albumentations_paper}} proposed by the reviewer. The new results in Supp. Mat. Section S3 confirm our previous results that segment-level augmentation is a better strategy than image-level augmentation for trademark retrieval.

\input{Albumentations_table}


\noindent\textbf{E2 - \Reight}: ``\textit{...limited to a particular logo recognition task}"

\Authors: We agree that our analysis is limited to logo retrieval. However, our method is a viable approach for reasoning about similarities at part levels and require transfer of knowledge or finding correspondences (e.g. affordances, partial shape similarity) at the level of object parts. This is an interesting research direction and we provide a discussion about this in Supp. Mat. Section S8.

\noindent\textbf{E3 - \Reight}: \textit{``... III.C.1, III.C.2 is not sufficiently clear."} \Authors: Sorry about the ambiguity. This was partially due to a mistake in notation (as noted by \Rfour). We've revised the notation and the text to make it more clear.


\noindent\textbf{E4 - \Reight}: \textit{I can only guess (without confidence) that you just simplify the Smooth AP by removing the ranking of inter-class samples. The Triplet Loss Adaptation seem to be straightforward for the problem. However, some sentences confuse the reader, for instance: "Optimizing the distances between dissimilar logo instances [...]."} \Authors: We've updated the text and improve the notation. We hope that it is more clear now.


\subsection{Minor Comments}
\noindent\hline
\vspace*{0.2cm}

\textbf{\Rfour}: \textit{``Omega notation has been used in two different variables.(logo and minibatch)"}. \textbf{\Rsix}: \textit{``There are many linguistic glitches here"}. \textbf{\Reight}: \textit{``The introduction of the data augmentation strategy at the beginning of the work creates the false first impression that it is primarily used to increase the "samples per class" value of the dataset. ... this should be better clarified in the III.A or elsewhere before introducing the methodology."} 

\Authors: Thank you for the suggestions and corrections. We've integrated them into the text and highlighted them in red.

\textbf{\Reight}: \textit{``...the location of Figures 2 and 3  (namely together with the text in double-column format) is not standard"} 

\Authors: We agree that such a layout is not ideal or pleasing to the eye; sorry for that. Though, this is allowed by the conference template and common in space scarcities.





==> ICPR2022 -- Logo Retrieval/sect_related_work.tex <==
\section{Related Work}

\subsection{Logo Retrieval}
Earlier studies in trademark retrieval \cite{TursunandKalkan} used hand-crafted features and deep features extracted using pre-trained networks and revealed that deep features obtained considerably better results. Perez \emph{et al.} \cite{Perez} improved the results by combining two CNNs trained on two different datasets. Later, Tursun \emph{et al.} \cite{Tursun2019} achieved impressive results by introducing different attention methods to reduce the effect of text regions, and in their most recent work \cite{Tursun2022}, they introduced different modifications and achieved state-of-the-art results. %Methods tested with the METU Trademark Dataset \cite{Kalkan} are mentioned to provide a more accurate comparison.

\subsection{Data Augmentation}
Data augmentation \cite{augmentation2, AugmentationSurvey} is an essential and well-known technique in deep learning to make networks more robust to variations in data.  Conventional augmentation methods perform geometric transformations such as zooming, flipping or cropping the entire image. Alternatively, adding noise, random erasing  or synthesizing training data \cite{ImageNet} are key approaches to improve overall model performance. Random Erasing \cite{RandomErasing} is a recently introduced method that obtains significant improvement on various recognition tasks. Although augmentation methods that focus on cutting and mixing windows \cite{CutMix,MixUp,imagemix}  rather than the whole image are not widely used, they have shown significant gains in performance. 

In logo retrieval, studies generally use conventional augmentation methods. For example, Tursun \emph{et al.} \cite{tursun2021learning} applied a reinforcement learning approach to learn an ensemble of test-time data augmentations for trademark retrieval. An exception to such an approach is the study by Tursun \emph{et al.} \cite{Tursun2019}, who proposed a method to remove text regions from logos while evaluating similarity. 

\subsection{Differentiable Ranking}

Image or logo retrieval are by definition ranking problems, though ranking is not differentiable. To address this limitation, many solutions have been proposed recently \cite{FastAP,BlackboxAP,Brown2020eccv}. These approaches mainly optimize Average Precision (AP) with different approximations: For example, Cakir \emph{et al.} \cite{FastAP} quantize distances between pairs of instances and use differentiable relaxations for these quantized distances. Rolinek \emph{et al.} \cite{BlackboxAP} consider non-differentiable ranking as a black box and use smoothing to estimate suitable gradients for training a network to rank. Finally, Brown \emph{et al.} \cite{Brown2020eccv} propose smoothing AP itself to use differentiable operations to train a deep network to rank.

%To solve this optimization problem, many influential methods \cite{song2016deep} are introduced with different approaches based on different approximations of AP metric. Significant progress have been achieved with different differentiable representations of AP \cite{FastAP}, smoothed differentiable approximations of AP \cite{BlackboxAP}, namely Smooth-AP \cite{Brown2020eccv}  loss leads to a further improvement.

These approximations have been mainly applied to standard retrieval benchmarks. In this paper, we show that differentiable ranking-based loss functions can lead to a performance improvement for logo retrieval as well.

\subsection{Summary}

Looking at the studies in the literature, we observe that \textbf{(1)} No study has performed segment-level augmentation either for logo retrieval or for general recognition or retrieval problems. The closest study for this research direction is the study by Tursun \emph{et al.} \cite{Tursun2019}, which just removed text regions in logos while evaluating similarity. \textbf{(2)} Promising deep learning approaches such as metric learning using e.g. Triplet Loss and differentiable ranking have not been employed for logo retrieval.

==> ICPR2022 -- Logo Retrieval/table_LLD.tex <==
\begin{table*}[hbt!]
\centering
\caption{\label{tab:LLDtable} Normalized Average Rank (NAR) and Recall@K values for data augmentation experiments from Albumentations library with ResNet architecture on LLD Dataset.}
 \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l l l l l | l l l l l l @{}}
\toprule
\textbf{} &
  \textbf{} &
  \textbf{Image Level} &
  \textbf{} &
   &
   & 
  \textbf{Segment Level} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
   \\ \midrule
\multicolumn{1}{c}{Resized Crop} &
  \multicolumn{1}{c}{Random Rotation} &
  \multicolumn{1}{c}{R. Horizontal Flip} &
  \multicolumn{1}{c}{Color Jitter} &
  \multicolumn{1}{|c}{S. Color Change} &
  \multicolumn{1}{c}{S. Rotation} &
  \multicolumn{1}{c}{S. Removal} &
  \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
  \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
  \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.044} &
  \multicolumn{1}{c}{0.556} &
  \multicolumn{1}{c}{0.724} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.068} &
  \multicolumn{1}{c}{0.527} &
  \multicolumn{1}{c}{0.679} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{0.038}} &
  \multicolumn{1}{c}{0.551} &
  \multicolumn{1}{c}{\textbf{0.738}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.039} &
  \multicolumn{1}{c}{0.551} &
  \multicolumn{1}{c}{0.719} \\ \midrule\midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.039} &
  \multicolumn{1}{c}{\textbf{0.581}} &
  \multicolumn{1}{c}{\textbf{0.738}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.058} &
  \multicolumn{1}{c}{0.527} &
  \multicolumn{1}{c}{0.687} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.051} &
  \multicolumn{1}{c}{0.532} &
  \multicolumn{1}{c}{0.704} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.054} &
  \multicolumn{1}{c}{0.561} &
  \multicolumn{1}{c}{0.719} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.056} &
  \multicolumn{1}{c}{0.517} &
  \multicolumn{1}{c}{0.704} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.068} &
  \multicolumn{1}{c}{0.507} &
  \multicolumn{1}{c}{0.684} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.064} &
  \multicolumn{1}{c}{0.536} &
  \multicolumn{1}{c}{0.684} \\ \bottomrule
  \addlinespace
\end{tabular}%
 }
\end{table*}



==> ICPR2022 -- Logo Retrieval/table_convnet.tex <==
\begin{table}[ht]
    \centering
    \caption{\label{tab:RebuttalConvNextTable} Experiments on the ConvNeXt architecture \cite{liu2022convnet} using Smooth-AP Loss. }
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        \multicolumn{1}{c}{Color C.} &
        \multicolumn{1}{c}{Rotation} &
        \multicolumn{1}{c}{Removal} &
        \multicolumn{1}{c}{\textbf{$p$}} &
        \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
        \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
        \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule \midrule
        \multicolumn{3}{c}{\textit{Baseline}} &
        \multicolumn{1}{c}{0} &
        \multicolumn{1}{c}{0.039} &
        \multicolumn{1}{c}{\textbf{0.438}} &
        \multicolumn{1}{c}{0.704}  \\ \midrule \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{\textbf{0.039}} &
        \multicolumn{1}{c}{0.413} &
        \multicolumn{1}{c}{\textbf{0.709}}  \\ \midrule
         \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.041} &
        \multicolumn{1}{c}{0.413} &
        \multicolumn{1}{c}{0.694}  \\ \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.040} &
        \multicolumn{1}{c}{0.403} &
        \multicolumn{1}{c}{0.699} \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.046} &
        \multicolumn{1}{c}{0.379} &
        \multicolumn{1}{c}{0.661} \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.045} &
        \multicolumn{1}{c}{0.374} &
        \multicolumn{1}{c}{0.684} \\ \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.051} &
        \multicolumn{1}{c}{0.369} &
        \multicolumn{1}{c}{0.655} \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.055} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{0.615} \\ \midrule
         \bottomrule
        \addlinespace
        \end{tabular}
    \end{table}

==> ICPR2022 -- Logo Retrieval/table_more_augmentation.tex <==
\begin{table*}[hbt!]
\centering
\caption{\label{tab:albumentations} Normalized Average Rank (NAR) and Recall@K values for data augmentation experiments from Albumentations Library with Smooth-AP Loss on ResNet.}
 \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l l l l l | l l l l l l @{}}
\toprule
\textbf{} &
  \textbf{} &
  \textbf{Image Level} &
  \textbf{} &
   &
   & 
  \textbf{Segment Level} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
   \\ \midrule
\multicolumn{1}{c}{Resized Crop} &
  \multicolumn{1}{c}{Cutout} &
  \multicolumn{1}{c}{Elastic Transform} &
  \multicolumn{1}{c}{Channel Shuffle} &
  \multicolumn{1}{|c}{S. Color Change} &
  \multicolumn{1}{c}{S. Rotation} &
  \multicolumn{1}{c}{S. Removal} &
  \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
  \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
  \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
  \multicolumn{7}{c}{\textit{Baseline}} &
  \multicolumn{1}{c}{0.102} &
  \multicolumn{1}{c}{0.310} &
  \multicolumn{1}{c}{0.536} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.052} &
  \multicolumn{1}{c}{0.325} &
  \multicolumn{1}{c}{0.581} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.060} &
  \multicolumn{1}{c}{\textbf{0.379}} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.0451} &
  \multicolumn{1}{c}{0.344} &
  \multicolumn{1}{c}{0.596} \\ \midrule\midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{0.040}} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.610} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.344} &
  \multicolumn{1}{c}{0.601} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.048} &
  \multicolumn{1}{c}{0.339} &
  \multicolumn{1}{c}{0.596} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{0.050} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.586} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.046} &
  \multicolumn{1}{c}{{0.374}} &
  \multicolumn{1}{c}{\textbf{0.625}} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.044} &
  \multicolumn{1}{c}{0.354} &
  \multicolumn{1}{c}{0.591} \\ \midrule
\multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} &
  \multicolumn{1}{c}{0.047} &
  \multicolumn{1}{c}{0.374} &
  \multicolumn{1}{c}{0.605} \\ \bottomrule
  \addlinespace
\end{tabular}%
 }
\end{table*}



==> ICPR2022 -- Logo Retrieval/time_complexity.tex <==
\begin{table}[ht]
    \centering
    \caption{\label{tab:RebuttalTimeComplexity} Time spent on different steps of segment-level and image-level augmentation.}
    \begin{tabular}{@{}lll@{}}
        \toprule
        \multicolumn{1}{c}{\textbf{Method}} &
        \multicolumn{1}{c}{\textbf{Segmentation}} &
        \multicolumn{1}{c}{\textbf{Transformation}} \\ \midrule\midrule
        \multicolumn{1}{c}{Color Jitter} &
        \multicolumn{1}{c}{-} &
        \multicolumn{1}{c}{1.2ms} \\ \midrule
        \multicolumn{1}{c}{R. Horizontal Flip} &
        \multicolumn{1}{c}{-} &
        \multicolumn{1}{c}{2.8ms } \\ \midrule \midrule
        \multicolumn{1}{c}{Segment Color} &
        \multicolumn{1}{c}{0.4ms} &
        \multicolumn{1}{c}{2.4ms} \\ \midrule
        \multicolumn{1}{c}{Segment Removal} &
        \multicolumn{1}{c}{0.4ms} &
        \multicolumn{1}{c}{4.3ms} \\  \midrule
        \multicolumn{1}{c}{Segment Rotation} &
        \multicolumn{1}{c}{0.4ms} &
        \multicolumn{1}{c}{14.0ms} \\
         \bottomrule
        \addlinespace
        \end{tabular}
\end{table}

% \begin{table}[ht]
%     \centering
%     \caption{ Test.}
%     \begin{tabular}{llll}
%         \toprule
%         \textbf{Segment-level Augmentation} &
%         \textbf{Time} &
%         \textbf{Image-level Augmentation} & 
%         \textbf{Time} \\ \midrule
%         %\bottomrule
%         \addlinespace
%     \end{tabular}
% \end{table}

==> ICPR2022 -- Logo Retrieval/tmp/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> ICPR2022 -- Logo Retrieval/tmp/tablo.tex <==
\begin{table*}[ht]
    \centering
    \caption{\label{tab:RankingLossesTable} Normalized Average Rank (NAR) and Recall values for Smooth AP and Triplet Loss adaptations.}
        \begin{tabular}{@{}lllllll@{}}
        \toprule
        \textbf{} &
          \textbf{Applied Segment Based Augmentation} &
          \textbf{} &
          \textbf{} &
          \textbf{} &
          \textbf{} &
          \textbf{} 
          \\
          \midrule
        \multicolumn{1}{c}{S. Color Change} &
        \multicolumn{1}{c}{S. Rotation} &
        \multicolumn{1}{c}{S. Removal} &
        \multicolumn{1}{c}{\textbf{Probability}} &
        \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
        \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
        \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{\textbf{0.040}} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{\textbf{0.610}} &  \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.043} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{0.601} &  \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{0.325} &
        \multicolumn{1}{c}{0.566} &  \midrule
         \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.601} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{\textbf{0.369}} &
        \multicolumn{1}{c}{0.591} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.060} &
        \multicolumn{1}{c}{0.330} &
        \multicolumn{1}{c}{0.556} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.339} &
        \multicolumn{1}{c}{0.596} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.571} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.591} &
         \bottomrule
        \addlinespace
        \end{tabular}
    \end{table*}

==> sect_rebuttal.tex <==



\section*{Authors' Response}

We thank all the reviewers for their valuable feedback. To summarize: The reviewers found our paper \textit{``well-motivated''} (\Rfour, \Rseven), \textit{``well-organized''} (\Rseven), \textit{``well-written''} (\Reight), containing \textit{``valuable ideas''} (\Rfour), and \textit{``interesting''} (\Reight) and noted that \textit{``experimental results demonstrate the effectiveness of the proposed strategy"} (\Rseven). The reviewers had concerns about the novelty of the ideas as well as the significance of the results. Moreover, they requested more analysis and a discussion of the limitations. 

We've addressed all reviewer comments and the quality of our paper improved significantly. To be specific, in addition to updating the text to clarify ambiguous points, we've conducted new experiments and we report positive results on another dataset ({LLD - Large Logo Dataset} \cite{sage2017logodataset} -- see item A3), with a more recent, stronger and fast backbone ({ConvNeXt} architecture \cite{liu2022convnet} -- see item {C1}), and provide a running-time analysis (C5), an analysis of the effect of text (C2), visual results (A2\&C6) and more discussion. In the following, we only summarize our changes and respond to the comments provided by the reviewers. Due to space limitations, the new results are provided in the supplementary material, with pointers placed in the main text.

\subsection{Common Concerns}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{A1. Simplicity of the Contribution.} 
\Rsix: \textit{``[t]he contribution and novelty of this paper are limited since the authors propose a standard application of well-known methods according to a classic algorithmic scheme (the proposed techniques are simple and already proposed in the literature)"}. \Reight: \textit{``idea of the proposed "segment level" augmentation appears more as an engineering, rather than a scientific contribution"}.

\Authors: We respectfully disagree with the reviewers on the requirement that a paper's methodology should be sophisticated or non-engineered: (i) [Computer] Science makes progress by putting together existing tools and methods in novel ways for solving problems, generally improving some performance measures while doing so. In our case, we do use existing tools (segmentation, augmentation) but propose a novel idea for combining them for solving an existing problem with a significantly better performance. (ii) An `engineering' approach can be scientific if the engineered solution is novel. (iii) There exist similar papers at top conferences (``Copy-paste networks...",  ICCV2017 \cite{lee2019copy} ; ``Cut, paste and learn...", ICCV2019 \cite{dwibedi2017cut}; ``Simple copy-paste ...", CVPR2021 \cite{ghiasi2021simple}) that propose ``simple'' and ``engineered'' augmentation methods or analyze them. Such papers are scientific contributions as they contribute to the progress of [Computer] Science by bringing together existing tools in new ways or by analyzing what's not been known before. We strongly believe that our paper is similar, its contributions are scientific and our novel idea deserves to be seen by the community. Moreover, our novel way of performing \& analyzing segment-level augmentation has strong potential for inspiring more granular augmentation strategies than what's generally used in the literature (see also E2 \& Supp. Mat. Section S8-C).

\noindent\textbf{A2. Quality and Explanation of segmentation.}

\textbf{\Rfour}: \textit{``...quantitative results and performance of segmentation quality are not given"}. \textbf{\Rseven}: \textit{... segmentation errors, limitations and errors should be discussed.}

\Authors: We thank the reviewers for highlighting this important point. Logos are simplistic images composed of regions that are generally homogeneous in color. Therefore, an off-the-shelf simple segmentation algorithm works well for most logos (see Supp. Mat. Section S4 for some examples). Logo segmentation can produce spurious segments especially on regions which have strong color gradients. However, such infrequent cases are not a problem for us because segments corresponding to over-segmentation or under-segmentation do function as segment-level augmentation and this is still useful for training. We provide a discussion about this in  Supp. Mat. Section S4.

%The reviewers raise an important point, and we were unable to analyze this in the paper due to space limitations. As the logo datasets do not have segment We note that \renkli{...} Moreover, even when the segmentation methods produces faulty segments, such faulty (broken) segments do function as sub-segment level augmentation and this is not necessarily a negative problem for training. 

\noindent\textbf{A3. Other Datasets}

\textbf{\Rfour}: \textit{``I encourage the authors to point out the performance of their method on more benchmark datasets."}

\textbf{\Rsix}: \textit{``... Please conduct more experiments on other recent datasets."}

\Authors: With this revision, we've performed experiments with the {LLD - Large Logo Dataset} {\cite{sage2017logodataset}}. Our results (Supp. Mat. Section S2) confirm that the performing segment-level augmentation is a working strategy for learning better representations for trademark similarity. These results are obtained without any hyper-parameter tuning and we anticipate the gap to widen if they are tuned.

\input{LLD_table}
\subsection{Specific Concerns of \Rfour}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{B1 - \Rfour}:  \textit{``contributions of the paper are not clearly stated, so the novelty remains somewhat questionable."}

\Authors: The last two paragraphs of Introduction state our contributions as follows (truncated to save space): 

``\textit{Main Contributions.} Our contributions are as follows:
\begin{itemize}
    \item We propose a segment-level augmentation for producing artificial similarities between logos. To the best of our knowledge, ours is the first to introduce segment-level augmentation in deep learning. [...]
    
    \item To showcase the use of such a tool to generate artificially similar logos, we use data-hungry deep learning methods, namely, Triplet Loss \cite{weinberger2009distance} and Smooth AP \cite{Brown2020eccv}, [...]"
\end{itemize}

\noindent\textbf{B2 - \Rfour}: \textit{``...table I and table II are not evident in order to demonstrate the performance. What are the chosen hyperparameters?"}

\Authors: In Table I, we see the effect of applying ranking/comparison-based losses for logo retrieval. We see that both Triplet Loss and Smooth-AP Loss do significantly improve over the baseline. Although these results are new for logo retrieval, the methods are not novel for our paper. In Table II, we show that applying image-level augmentation improves logo retrieval performance; though we obtain better gain with our proposed way of performing segment-level augmentation. The hyper-parameters are provided in detail in Section IV.A.2.

\subsection{Specific Concerns of \Rsix}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{C1 - \Rsix}: \textit{``...the authors should compare their contribution with recent deep networks."}
\input{ConvNext_table}
\Authors: We now compare our method with a very recent CNN architecture, namely, ConvNeXt \cite{liu2022convnet}. The new results in Supp. Mat. Section S1 confirm our hypothesis that segment-level augmentation performs on par or improves logo retrieval performance. Our ongoing experiments with ResNext, which could not be completed because ResNext is slower than ResNet or ConvNeXt, also promise significant gain in favor of using segment-level augmentation (results will be included in the camera-ready version).

\noindent\textbf{C2 - \Rsix}: \textit{``...justify why ResNet performs worse on logos having text content in IV-B Experiment 1. ... give qualitative and quantitative performance analysis of this observation"}

\Authors: We now provide both qualitative \& quantitative results on this in Supp. Mat. Section S5, and provide a discussion.

\noindent\textbf{C3 - \Rsix}: \textit{``...why certain transformations in the data augmentation step are more performant when applying Triplet Loss, while other are better when using Smooth AP."}.

\Authors: This is an important point and we now provide a discussion on this in Supp. Mat. Section S8. To provide a summary here: Smooth AP and Triplet Loss incur different inductive ranking biases and this leads to different overall behaviors for the methods.

\noindent\textbf{C4 - \Rsix}: \textit{``...best value of p depends on the type of used transformation and the computed performance evaluation metric."}.

\Authors: The reviewer is right about this point. However, different augmentations incur different biases and it is not surprising that they contribute to performance differently and with different selection probabilities. We now provide a discussion about this in Supp. Mat. Section S8.

\noindent\textbf{C5 - \Rsix}: \textit{``...discussion on the complexity (e.g. training time and retrieval response) is missing."}

\Authors: We now provide a running-time analysis in Supp. Mat. Section S7.

\noindent\textbf{C6 - \Rsix}: \textit{``The authors should present an error analysis to find the reasons behind the incurred errors by analyzing correlations between the different scenarios."}

\Authors: We now provide more qualitative analysis in Supp. Mat. Sections S4 and S6 on failure cases as well and provide a discussion for potential reasons.

\noindent\textbf{C7 - \Rsix:} \textit{``The Triplet Loss function requires preparing a database done by triplets of images, limiting its application to the existing publicly available datasets."}

\Authors: Taking samples from a class as anchors \& positive samples, and samples from other classes as negative samples, applying Triplet Loss is actually very straightforward and can be applied to any classification or retrieval problem. This can be easily done on the run while sampling a batch without preparing a separate dataset.

\subsection{Specific Concerns of \Rseven}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{D1 - \Rseven}: \textit{"...Please further discuss the performance of triplet loss and smooth AP loss in Table \ref{tab:RankingLossesTable}}

\Authors: We now provide a discussion on this in Supp. Mat. Section S6. To provide a summary here: Smooth AP and Triplet Loss incur different inductive ranking biases and this leads to different overall behaviors for the methods.

\subsection{Specific Concerns of \Reight}
\noindent\hline
\vspace*{0.2cm}

\noindent\textbf{E1 - \Reight:} ``\textit{The variety of image-level augmentation techniques, which were used for comparison, is insufficient and the selected techniques themselves are trivial. To improve the impact of that contribution a better comparison with other techniques should be performed. For instance, the are public implementations [1,2]."}

\Authors: We now compare with three more commonly-used image-level augmentation methods (namely, {Cutout, Elastic Transform and Channel Shuffle}) from the library  {\cite{albumentations_paper}} proposed by the reviewer. The new results in Supp. Mat. Section S3 confirm our previous results that segment-level augmentation is a better strategy than image-level augmentation for trademark retrieval.

\input{Albumentations_table}


\noindent\textbf{E2 - \Reight}: ``\textit{...limited to a particular logo recognition task}"

\Authors: We agree that our analysis is limited to logo retrieval. However, our method is a viable approach for reasoning about similarities at part levels and require transfer of knowledge or finding correspondences (e.g. affordances, partial shape similarity) at the level of object parts. This is an interesting research direction and we provide a discussion about this in Supp. Mat. Section S8.

\noindent\textbf{E3 - \Reight}: \textit{``... III.C.1, III.C.2 is not sufficiently clear."} \Authors: Sorry about the ambiguity. This was partially due to a mistake in notation (as noted by \Rfour). We've revised the notation and the text to make it more clear.


\noindent\textbf{E4 - \Reight}: \textit{I can only guess (without confidence) that you just simplify the Smooth AP by removing the ranking of inter-class samples. The Triplet Loss Adaptation seem to be straightforward for the problem. However, some sentences confuse the reader, for instance: "Optimizing the distances between dissimilar logo instances [...]."} \Authors: We've updated the text and improve the notation. We hope that it is more clear now.


\subsection{Minor Comments}
\noindent\hline
\vspace*{0.2cm}

\textbf{\Rfour}: \textit{``Omega notation has been used in two different variables.(logo and minibatch)"}. \textbf{\Rsix}: \textit{``There are many linguistic glitches here"}. \textbf{\Reight}: \textit{``The introduction of the data augmentation strategy at the beginning of the work creates the false first impression that it is primarily used to increase the "samples per class" value of the dataset. ... this should be better clarified in the III.A or elsewhere before introducing the methodology."} 

\Authors: Thank you for the suggestions and corrections. We've integrated them into the text and highlighted them in red.

\textbf{\Reight}: \textit{``...the location of Figures 2 and 3  (namely together with the text in double-column format) is not standard"} 

\Authors: We agree that such a layout is not ideal or pleasing to the eye; sorry for that. Though, this is allowed by the conference template and common in space scarcities.





==> tmp/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tmp/tablo.tex <==
\begin{table*}[ht]
    \centering
    \caption{\label{tab:RankingLossesTable} Normalized Average Rank (NAR) and Recall values for Smooth AP and Triplet Loss adaptations.}
        \begin{tabular}{@{}lllllll@{}}
        \toprule
        \textbf{} &
          \textbf{Applied Segment Based Augmentation} &
          \textbf{} &
          \textbf{} &
          \textbf{} &
          \textbf{} &
          \textbf{} 
          \\
          \midrule
        \multicolumn{1}{c}{S. Color Change} &
        \multicolumn{1}{c}{S. Rotation} &
        \multicolumn{1}{c}{S. Removal} &
        \multicolumn{1}{c}{\textbf{Probability}} &
        \multicolumn{1}{c}{\textbf{NAR $\downarrow$}} &
        \multicolumn{1}{c}{\textbf{R@1 $\uparrow$}} &
        \multicolumn{1}{c}{\textbf{R@8 $\uparrow$}} \\ \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{\textbf{0.040}} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{\textbf{0.610}} &  \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.043} &
        \multicolumn{1}{c}{0.354} &
        \multicolumn{1}{c}{0.601} &  \midrule
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{0.325} &
        \multicolumn{1}{c}{0.566} &  \midrule
         \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.601} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.049} &
        \multicolumn{1}{c}{\textbf{0.369}} &
        \multicolumn{1}{c}{0.591} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.060} &
        \multicolumn{1}{c}{0.330} &
        \multicolumn{1}{c}{0.556} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.5} &
        \multicolumn{1}{c}{0.048} &
        \multicolumn{1}{c}{0.339} &
        \multicolumn{1}{c}{0.596} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{0.75} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.571} &  \midrule
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{\checkmark} &
        \multicolumn{1}{c}{1.0} &
        \multicolumn{1}{c}{0.047} &
        \multicolumn{1}{c}{0.344} &
        \multicolumn{1}{c}{0.591} &
         \bottomrule
        \addlinespace
        \end{tabular}
    \end{table*}
